Bayesian Classification and Regression with High Dimensional Features

This thesis responds to the challenges of using a large number, such as thousands, of features in regression and classification problems. There are two situations where such high dimensional features arise. One is when high dimensional measurements are available, for example, gene expression data produced by microarray techniques. For computational or other reasons, people may select only a small subset of features when modelling such data, by looking at how relevant the features are to predicting the response, based on some measure such as correlation with the response in the training data. Although it is used very commonly, this procedure will make the response appear more predictable than it actually is. In Chapter 2, we propose a Bayesian method to avoid this selection bias, with application to naive Bayes models and mixture models. High dimensional features also arise when we consider high-order interactions. The number of parameters will increase exponentially with the order considered. In Chapter 3, we propose a method for compressing a group of parameters into a single one, by exploiting the fact that many predictor variables derived from high-order interactions have the same values for all the training cases. The number of compressed parameters may have converged before considering the highest possible order. We apply this compression method to logistic sequence prediction models and logistic classification models. We use both simulated data and real data to test our methods in both chapters.

==> colon-pred-cv.tex <==
\begin{tabular}
{ccccccccccc}
\hline
\multicolumn{11}{c}{Average Minus Log Likelihood}\\ 
\hline
  Corrected& 0.499& 0.601& 0.369& 0.516& 0.511& 0.514& 0.587& 0.476& 0.426& 0.605\\ 
Uncorrected& 0.602& 0.734& 0.371& 0.594& 0.628& 0.571& 0.665& 0.542& 0.505& 0.721\\ 
\hline
\hline
\multicolumn{11}{c}{Mean Square Error}\\ 
\hline
  Corrected& 0.144& 0.178& 0.113& 0.152& 0.141& 0.159& 0.194& 0.154& 0.114& 0.147\\ 
Uncorrected& 0.151& 0.186& 0.110& 0.158& 0.143& 0.160& 0.200& 0.164& 0.118& 0.145\\ 
\hline
\end{tabular}


==> fig-bnnm <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
6 3900 1612 4275 1837
4 0 0 50 0 0 20 0.0000 4 135 150 3900 1762 x\001
4 0 0 50 0 0 12 0.0000 4 135 90 4125 1837 1\001
-6
6 8925 1500 9300 1800
4 0 0 50 0 0 20 0.0000 4 135 150 8925 1650 x\001
4 0 0 50 0 0 12 0.0000 4 135 90 9150 1725 p\001
-6
6 6000 4455 6315 4725
4 0 0 50 0 32 20 0.0000 4 210 165 6000 4650 q\001
4 0 0 50 0 0 12 0.0000 4 135 90 6225 4725 1\001
-6
6 11235 4335 11550 4650
4 0 0 50 0 32 20 0.0000 4 210 165 11235 4530 q\001
4 0 0 50 0 0 12 0.0000 4 135 90 11460 4605 p\001
-6
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 1 2
	0 0 1.00 60.00 120.00
	 5475 3375 6000 4350
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 1 2
	0 0 1.00 60.00 120.00
	 5568 5840 6093 4865
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 1 2
	0 0 1.00 60.00 120.00
	 10650 3375 11175 4350
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 1 2
	0 0 1.00 60.00 120.00
	 10685 5699 11210 4724
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 5025 3150 4350 3150
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 5100 5850 4425 5850
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 10125 3150 9450 3150
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 10200 5775 9525 5775
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 7425 4500 5700 3375
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 7425 4650 5700 5850
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 7773 4642 10248 5617
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 7800 4500 10200 3300
2 1 1 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 2250 4500 9375 4500
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 1425 4500 2100 4500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 2700 3300 3375 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 2700 5925 3375 5925
4 0 0 50 0 0 20 0.0000 4 210 150 2325 1770 y\001
4 0 0 50 0 0 20 0.0000 4 210 150 4012 2505 0\001
4 0 0 50 0 0 20 0.0000 4 210 150 2325 2505 0\001
4 0 0 50 0 0 12 0.0000 4 135 225 5325 3375  01\001
4 0 0 50 0 0 12 0.0000 4 135 225 5325 6000  11\001
4 0 0 50 0 0 20 0.0000 4 210 150 4012 4905 0\001
4 0 0 50 0 0 20 0.0000 4 210 150 2325 4905 1\001
4 0 0 50 0 0 20 0.0000 4 210 150 4012 5580 1\001
4 0 0 50 0 0 20 0.0000 4 210 150 2325 5580 1\001
4 0 0 50 0 0 20 0.0000 4 210 150 4012 6255 1\001
4 0 0 50 0 0 20 0.0000 4 210 150 2325 6255 1\001
4 0 0 50 0 0 20 0.0000 4 210 150 4012 6930 1\001
4 0 0 50 0 0 20 0.0000 4 210 150 2325 6930 1\001
4 0 0 50 0 0 20 0.0000 4 210 150 4012 4267 1\001
4 0 0 50 0 0 20 0.0000 4 210 150 2325 4267 0\001
4 0 0 50 0 0 20 0.0000 4 210 150 4012 3705 0\001
4 0 0 50 0 0 20 0.0000 4 210 150 2325 3705 0\001
4 0 0 50 0 0 20 0.0000 4 210 150 4012 3105 0\001
4 0 0 50 0 0 20 0.0000 4 210 150 2325 3105 0\001
4 0 0 50 0 0 12 0.0000 4 180 225 10425 3300  0p\001
4 0 0 50 0 0 12 0.0000 4 180 225 10425 5925  1p\001
4 0 0 50 0 32 20 0.0000 4 285 165 10275 5850 f\001
4 0 0 50 0 32 20 0.0000 4 285 165 10275 3225 f\001
4 0 0 50 0 0 20 0.0000 4 210 150 9037 2430 0\001
4 0 0 50 0 0 20 0.0000 4 210 150 9037 4830 0\001
4 0 0 50 0 0 20 0.0000 4 210 150 9037 5505 0\001
4 0 0 50 0 0 20 0.0000 4 210 150 9037 6180 1\001
4 0 0 50 0 0 20 0.0000 4 210 150 9037 6855 1\001
4 0 0 50 0 0 20 0.0000 4 210 150 9037 4192 1\001
4 0 0 50 0 0 20 0.0000 4 210 150 9037 3630 1\001
4 0 0 50 0 0 20 0.0000 4 210 150 9037 3030 0\001
4 0 0 50 0 32 20 0.0000 4 285 165 5175 5925 f\001
4 0 0 50 0 32 20 0.0000 4 285 165 5175 3300 f\001
4 0 0 50 0 0 26 0.0000 4 45 735 6300 1725 ... ...\001
4 0 0 50 0 32 20 0.0000 4 150 195 7500 4650 a\001
4 0 0 50 0 32 20 0.0000 4 225 210 1125 4575 y\001


==> format.tex <==
\usepackage{fancyhdr}
\usepackage{cite}
\usepackage{epic}
\usepackage{psfig}
\usepackage{latexsym}
\usepackage{amsmath}
\usepackage[usenames]{color}
\usepackage[dvips]{epsfig}
\usepackage{graphicx}
\usepackage{verbatim}
\usepackage{setspace} 

\renewcommand{\cleardoublepage}{\newpage}

\topmargin -0.2in 
\textheight 8.7in
\textwidth 6.5in
\oddsidemargin 0.31in
\evensidemargin -0.18in


\pagestyle{fancy}
\fancyhf{}
\renewcommand\headrulewidth{0.2pt}

%if for 2-sided
\fancyhead[RO,LE]{\bfseries\thepage}


\fancyhead[C]{\small \textit{{\thechapter}\ \chaptername}}

\fancypagestyle{plain}{ 
\fancyhf{} 
\fancyfoot[C]{\bfseries\thepage} 
\renewcommand\headrulewidth{0pt} 
}

\newenvironment{preliminary}%
  {\pagestyle{plain}\pagenumbering{roman}}%
  {\cleardoublepage}

\newenvironment{thesis}
{\pagestyle{fancy}\pagenumbering{arabic}\doublespacing}
{}

%%%%%%%%%%%%%%%%%%%%%%%%%%%New Command Area%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand{\ceil}[1]{\lceil #1 \rceil}
\newcommand{\Var}{\mbox{Var}}
\newcommand{\Cov}{\mbox{Cov}}

\newcommand{\Cor}{\mbox{Cor}} 

\newcommand{\COR}{\mbox{COR}}

\newcommand{\COV}{\mbox{COV}} 

\newcommand{\E}{\mbox{E}}

\newcommand{\PP}{\mbox{P}} 

\newcommand{\mc}{\multicolumn}

\newcommand{\mychoose}[2]{\Big(\begin{tabular}{c} $#1$ \\[-9pt] $#2$
\end{tabular}\Big)}

\newcommand{\given}{\ | \ }
\newcommand{\zi}{z^{(i)}}
\newcommand{\zz}{z^{(1)},\cdots,z^{(n)}}

\newcommand{\itb}{\begin{itemize}}
\newcommand{\itn}{\end{itemize}}
\newcommand{\nmn}{\end{enumerate}}
\newcommand{\nmb}{\begin{enumerate}}
\newcommand{\ctb}{\begin{center}}
\newcommand{\ctn}{\end{center}}
\newcommand{\tb}{\begin{center}\Large \bf}
\newcommand{\tn}{\end{center}}
\newcommand{\arb}{\begin{array}}
\newcommand{\qrn}{\end{array}}
\newcommand{\tblb}{\begin{tabular}}
\newcommand{\tbln}{\end{tabular}}
\newcommand{\fb}{\begin{figure}}
\newcommand{\fn}{\end{figure}}

\def\bern{\mbox{Bernoulli}\,}
\def\betad{\mbox{Beta}\,}

\def\ybar{\overline{y}}

\def\beq{\noindent \begin{eqnarray}}
\def\eeq{\end{eqnarray}}

\def\beqs {\noindent \begin{eqnarray*}}
\def\eeqs {\end{eqnarray*}}


\def\mb#1{\mbox{\boldmath $#1$}}

\def\A{\mathcal{A}}
\def\v{\mb v}
\def\w{\mb w}
\def\x{\mb x}
\def\z{\mb z}
\def\thetab{\mb \theta}
\def\phib{\mb \phi}
\def\etab{\mb \eta}
\def\betab{\mb \beta}
\def\epsilonb{\mb \epsilon}
\def\Psib{\mb \Psi}
\def\IID{
 \,\begin{array}{cc} \\[-20pt] \mbox{\tiny IID} \\[-15pt] \sim \end{array}\,}

\def\trn{^{\mbox{\tiny train}}}
\def\nulu{^{\mbox{~}}}

\def \cc {\mbox{Cauchy}}

\def \lldots {\ \ldots \ }

\def \trainingdata {\mathcal{D}}

\def \P {\mathcal{P}}

\def \EP {\mathcal{E}}

%\def \sigmaa {\sigma_g^{(1)}}

%\def \sigmaa {\sigma_g^{(1)}}

\def \sigmaa {\Sigma_1}
\def \sigmab {\Sigma_2}

\def \s {s_g}
\def \st {s^t_g}



==> naive-tab.tex <==
\begin{tabular}
{@{}c|@{}rcc|@{}rcc|rcc|rcc@{}}
         & \multicolumn{6}{c|}{\bf  1 feature selected out of 10000 } & \multicolumn{6}{c}{\bf  10 features selected out of 10000 } \\[5pt] 
         & \multicolumn{3}{c}{Corrected} & \multicolumn{3}{c|}{Uncorrected} & \multicolumn{3}{c}{Corrected} & \multicolumn{3}{c}{Uncorrected} \\[5pt] 
C & \mbox{~~~}\#\mbox{~} & \small{Pred} & \small{Actual} & \mbox{~~~}\#\mbox{~} & \small{Pred} & \small{Actual} & \mbox{~~}\#\mbox{~} & \small{Pred} & \small{Actual} & \mbox{~~}\#\mbox{~} & \small{Pred} & \small{Actual} \\[5pt] 
0 &    0 &    -- &    -- &    0 &    -- &    -- &    0 &    -- &    -- &  237 & 0.046 & 0.312 \\ 
1 &    0 &    -- &    -- &    0 &    -- &    -- &    3 & 0.174 & 0.000 &  349 & 0.149 & 0.444 \\ 
2 &    0 &    -- &    -- &    0 &    -- &    -- &  126 & 0.270 & 0.294 &   68 & 0.249 & 0.500 \\ 
3 &    0 &    -- &    -- & 1346 & 0.384 & 0.461 &  467 & 0.360 & 0.420 &  300 & 0.360 & 0.443 \\ 
4 & 1346 & 0.446 & 0.461 &    0 &    -- &    -- &  566 & 0.462 & 0.461 &  189 & 0.443 & 0.487 \\ 
5 &    0 &    -- &    -- &    0 &    -- &    -- &  461 & 0.554 & 0.566 &   48 & 0.546 & 0.417 \\ 
6 &  654 & 0.611 & 0.581 &    0 &    -- &    -- &  276 & 0.643 & 0.616 &  238 & 0.650 & 0.588 \\ 
7 &    0 &    -- &    -- &  654 & 0.736 & 0.581 &   97 & 0.733 & 0.742 &  180 & 0.737 & 0.567 \\ 
8 &    0 &    -- &    -- &    0 &    -- &    -- &    4 & 0.825 & 0.750 &  192 & 0.864 & 0.609 \\ 
9 &    0 &    -- &    -- &    0 &    -- &    -- &    0 &    -- &    -- &  199 & 0.943 & 0.668 \\ 
\end{tabular}

\vspace*{0.45in}
\begin{tabular}
{@{}c|@{}rcc|@{}rcc|rcc|rcc@{}}
         & \multicolumn{6}{c|}{\bf  100 features selected out of 10000 } & \multicolumn{6}{c}{\bf  1000 features selected out of 10000 } \\[5pt] 
         & \multicolumn{3}{c}{Corrected} & \multicolumn{3}{c|}{Uncorrected} & \multicolumn{3}{c}{Corrected} & \multicolumn{3}{c}{Uncorrected} \\[5pt] 
C & \mbox{~~~}\#\mbox{~} & \small{Pred} & \small{Actual} & \mbox{~~~}\#\mbox{~} & \small{Pred} & \small{Actual} & \mbox{~~}\#\mbox{~} & \small{Pred} & \small{Actual} & \mbox{~~}\#\mbox{~} & \small{Pred} & \small{Actual} \\[5pt] 
0 &  155 & 0.067 & 0.077 &  717 & 0.017 & 0.199 &  774 & 0.018 & 0.027 &  954 & 0.004 & 0.066 \\ 
1 &  247 & 0.151 & 0.162 &  133 & 0.150 & 0.391 &   97 & 0.143 & 0.165 &   28 & 0.149 & 0.500 \\ 
2 &  220 & 0.247 & 0.286 &   70 & 0.251 & 0.429 &   63 & 0.243 & 0.302 &   13 & 0.248 & 0.846 \\ 
3 &  225 & 0.352 & 0.356 &   68 & 0.351 & 0.515 &   48 & 0.346 & 0.438 &   17 & 0.349 & 0.412 \\ 
4 &  237 & 0.450 & 0.494 &   58 & 0.451 & 0.500 &   45 & 0.446 & 0.600 &   14 & 0.449 & 0.786 \\ 
5 &  227 & 0.545 & 0.586 &   78 & 0.552 & 0.603 &   44 & 0.547 & 0.614 &   16 & 0.546 & 0.375 \\ 
6 &  202 & 0.650 & 0.728 &   77 & 0.654 & 0.532 &   53 & 0.647 & 0.698 &   16 & 0.667 & 0.812 \\ 
7 &  214 & 0.749 & 0.785 &   80 & 0.746 & 0.662 &   81 & 0.755 & 0.815 &   22 & 0.751 & 0.636 \\ 
8 &  182 & 0.847 & 0.857 &   98 & 0.852 & 0.633 &  124 & 0.854 & 0.863 &   25 & 0.865 & 0.560 \\ 
9 &   91 & 0.935 & 0.923 &  621 & 0.979 & 0.818 &  671 & 0.977 & 0.982 &  895 & 0.995 & 0.946 \\ 
\end{tabular}

\vspace*{0.45in}
\begin{tabular}[t]
{@{}c|@{}rcc@{}}
         & \multicolumn{3}{c}{\bf Complete data} \\[5pt] 
C & \mbox{~~~}\#\mbox{~} & \small{Pred} & \small{Actual} \\[5pt] 
0 &  964 & 0.004 & 0.006 \\ 
1 &   21 & 0.145 & 0.238 \\ 
2 &    8 & 0.246 & 0.375 \\ 
3 &   10 & 0.342 & 0.300 \\ 
4 &   12 & 0.436 & 0.500 \\ 
5 &    7 & 0.544 & 1.000 \\ 
6 &   20 & 0.656 & 1.000 \\ 
7 &   13 & 0.743 & 0.846 \\ 
8 &   22 & 0.851 & 0.818 \\ 
9 &  923 & 0.994 & 0.998 \\ 
\end{tabular}


==> slide_bias_jsm.tex <==
\input{head}
\newcommand{\tr}{^{\mbox{\tiny train}}}
\newcommand{\given}{\ |\ }
\def\IID{
 \,\begin{array}{cc} \\[-20pt] \mbox{\tiny IID} \\[-7pt] \sim \end{array}\,}
\slideframe{none}
%------------------------------------------------------- title
\begin{slide}
\tb \large Avoiding bias from feature selection \\
in regression and classification models\tn
\vspace{0.5in}
\ctb Longhai Li \ctn
\ctb Department of Statistics \\University of Toronto \ctn
\bigskip
\ctb Joint work with Radford Neal and Jianguo Zhang\ctn
\vfill

\ctb
Joint Statistical Meeting, Seattle, 9 Aug 2006
\ctn
\end{slide}

%-------------------------------------------------------slide2
\begin{slide}
\tb The Bias from Feature Selection \tn
\begin{itemize}
\item We want to predict a response $y$ using predictors $x_{1},\ldots,x_{p}$. \item When $p$ is big we may have to select a much smaller number, say $k$, of features to use due to computational or other reasons. 
\item We may decide to keep only the features having high correlation with $y$.
\item {\bf However}, this may result in overconfident prediction on test data.\\

\indent As an extreme example, even when {\bf all} the features are unrelated to $y$, there may seem to be strong correlations between $y$ and the selected features.
\end{itemize}
\end{slide}
%-------------------------------------------------------slide3
\begin{slide}
\tb Our approach to avoiding selection bias\tn
\begin{itemize}
\item {\bf General Idea}: Retain the information that $p-k$ features were discarded because of their weak correlation with the response.  
\item {\bf Joint modeling}: The response and the predictors are modeled jointly. Given the response $y$, perhaps some latent values $z$, and model parameters $\alpha$ and $\theta_1,\ldots,\theta_p$, the predictors are modeled to be independent:
$$
P(x_1,\cdots,x_p,y,z,\theta_1,\cdots,\theta_p,\alpha) = P(y,z,\alpha)\prod_{t=1}^p P(x_t\given y,z,\theta_t,\alpha)P(\theta_t\given \alpha)
$$
The graphical model for independent cases, $i=1,\ldots,n$:
\begin{center}
\includegraphics[height=1in,width=3in]{fig-gr-model}
\end{center}
\end{itemize}
\end{slide}
\begin{slide}
\tb Our approach to avoiding selection bias (continued) \tn
\small
\begin{itemize}
\item {\bf Feature Selection}: Suppose we discard a feature
$x\tr_t$ if it has sample correlation (COR)
with
$y\tr$ less than $\gamma$.\\
 Let $\mathcal{B}_\gamma=\{\tilde{x}: |\mbox{COR}(\tilde{x},y\tr)| < \gamma\}$ be the set of all possible such features.
\item {\bf Modified Likelihood function}: The likelihood function of $\alpha,z$ should be based on the selected features $x_1\tr,\ldots,x_k\tr$ and the fact, $\mathcal{S}$, that $p-k$ features are in set $\mathcal{B_\gamma}$. If we don't use latent values, this is:
\begin{eqnarray*}
\lefteqn{L(\alpha; y\tr,x\tr_1,\cdots,x\tr_k,\mathcal{S})}\\
&=& \left[\prod_{t=1}^k P(x\tr_t \given y\tr,\theta_t,\alpha)P(\theta_t\given \alpha)\right]\cdot P(\mathcal{S} \given \alpha,y\tr)\\
&=&\left[\prod_{t=1}^k P(x\tr_t \given y\tr,\theta_t,\alpha)P(\theta_t\given \alpha)\right]\cdot \left[P(x\tr_{k+1} \in \mathcal{B}_\gamma\given \alpha,y\tr)\right]^{p-k}
\end{eqnarray*}
Note that the probability in the last factor needs to be calculated only once regardless how many features are discarded, since $P(x_t\tr \in \mathcal{B}_\gamma \given \alpha, y\tr)$ is the same for all $t>k$.
\end{itemize}
\end{slide}
%-------------------------------------------------------slide4
\begin{slide}
\tb Binary naive Bayes Models \tn 
\begin{eqnarray*} 
   \phi_y &\sim& \mbox{Beta}(f_1,f_0)\\
    y^{(1)},\ldots,y^{(n)} \given \phi_y &\IID& \mbox{Bernoulli}(\phi_y)\\     
    \alpha &\sim& \mbox{Inverse-Gamma}(\alpha_0,\lambda_0)\\
    \theta_1,\ldots,\theta_p &\IID& \mbox{Uniform}(a_0,b_0)\\
    \phi_{0j},\phi_{1j}\ |\ \alpha,\theta_j &\IID&      \mbox{Beta}(\alpha\theta_j,\alpha(1-\theta_j)), \ \ \ \mbox{for } j=1,\ldots,p  \\   
    x^{(i)}_j\ |\ y^{(i)}, {\bf \phi}_{y^{(i)}} &\sim&
     \mbox{Bernoulli}(\phi_{y^{(i)}j}) ,\ \ \  \mbox{for }i=1,\ldots,n    
\end{eqnarray*}
Note that $\var( \phi_{yj}) = \theta_j(1-\theta_j)/\alpha+1$. When $\alpha$ is bigger, the $\phi_{0j}$ and $\phi_{1j}$ are more likely to be close, and feature $j$ is less likely to be correlated with the response $y$. Therefore $\alpha$ controls the overall degree of correlation between $y$ and the features.
\end{slide}
%-------------------------------------------------------slide5
\begin{slide}
\tb  Picture of the binary naive Bayes models  \tn
\begin{center}
\includegraphics[scale=0.57]{fig-bnnm}
\end{center}
\end{slide}
%-------------------------------------------------------slide6
\begin{slide}
\tb Training the models with bias correction \tn
\begin{itemize}
\item We use MCMC with $\alpha$ and $\theta_1,\ldots,\theta_k$ as the state
\item For $j=1,\cdots,k$, the posterior of $\theta_j$ given $\alpha$ is based only on $x_j\tr$ and the prior. $\phi_{0j}$ and $\phi_{1j}$ can be integrated away using the Polya urn scheme. 
\item The posterior of $\alpha$ is based on $x_1\tr,\ldots,x_k\tr$  as well as $\mathcal{S}$. Suppose we draw $\phi_{0j}$ and $\phi_{1j}$, $j=1,\ldots,k$ for temporary use, the posterior of $\alpha$ is:
\begin{eqnarray*}
\lefteqn{P(\alpha \given \mathcal{S}, \phi_{0j},\phi_{1j},j=1,\ldots,k)}\\ 
&=& P(\alpha)\left[\prod_{j=1}^k \prod_{y=0}^1\mbox{beta}(\phi_{yj};\alpha\theta_j,\alpha(1-\theta_j))\right] \cdot [P(x_{k+1}\tr\in \mathcal{B}_\gamma\given \alpha, y\tr)]^{p-k}
\end{eqnarray*}
where $\mathcal{B}_\gamma=\{\tilde{x}: |\mbox{COR}(\tilde{x},y\tr)| < \gamma\}$. 
\item Note that the adjustment factor is an increasing function of $\alpha$
\end{itemize}
\end{slide}
%-------------------------------------------------------slide7
\begin{slide}
\tb Evaluation of the adjustment factor \tn
\begin{itemize}
\item Evaluating the adjustment factor precisely is difficult. We need to sum the probability of feature $x_{k+1}\tr$ over all points in $\mathcal{B}_\gamma$ and integrate over $\theta_{k+1}$:
\begin{eqnarray*}
P(x\tr_{k+1}\in \mathcal{B}_\gamma\given \alpha, y\tr)
&=&\sum_{x\tr_{k+1}\in\mathcal{B}_\gamma}P(x\tr_{k+1}\given
\alpha,
y\tr)\\
&=&\int\!\sum_{x\tr_{k+1}\in\mathcal{B}_\gamma}\!P(x\tr_{k+1}\given
\alpha,\theta_{k+1}, y\tr)P(\theta_{k+1})d\theta_{k+1}
\end{eqnarray*}
\item For binary naive Bayes model, ways are available to do this faster:
       \begin{itemize}   
       \item $\mathcal{B}_\gamma$ is determined only by 
       $n_{01}=\sum_{i=1}^nI(y^{(i)}=0,x^{(i)}_{k+1}=1)$ and $n_{11}=\sum_{i=1}^n
       I(y^{(i)}=1,x^{(i)}_{k+1}=1)$
       \item $P(x\tr_{k+1} \given \alpha,\theta_{k+1},y\tr)$ is determined also only by $n_{01}$ and $n_{11}$. 
       \end{itemize}
\item Since we can evaluate the integrand for a particular $\theta_{k+1}$, then we can approximate the adjustment factor using Simpson's Rule.
\end{itemize}
\end{slide}
%-------------------------------------------------------slide8
\begin{slide}
\tb A Simulation Study \tn
\begin{itemize}
\item {\bf Generating the data set}: with $\alpha=400$,
$a_0=0$, $b_0=1$, and $p=10000$, we generated 350 cases with $y=1$ and 350 cases with $y=0$. From each group we chose 50 cases as the training data.
\item {\bf Training the model}: Priors used had $a_0=0,b_0=1$, $\alpha_0=5,\lambda_0=500$. 300 iterations of the Markov chain were run.
\item {\bf Feature selection}: Subsets of 1, 10, 100, 1000, and 2000 features were selected based on the absolute correlation with $y\tr$. 
\item {\bf Assessment}: After obtaining the predictive probabilities for the 600 test cases, we categorized them by the first decimal of predictive probabilities into 10 groups. Within each group, we calculated the average predictive probability and compared it with the actual fraction of class 1. \\
We also compared the posterior samples of $\alpha$ with the true value of 400. 
\end{itemize}
\end{slide}
%-------------------------------------------------------slide9
\begin{slide}
\tb Predictive probabilities for 600 test cases \tn
\small
\begin{center}
\begin{tabular}
{
 c   |  c       c       c   |   c       c       c   ||  c c
c}
\hline
    &   \mc{6}{c}{2000 Features Selected Out of 10000 (20\%)}                                         &   \mc{3}{c}{Complete Data Set}                    \\
\hline
    &   \mc{3}{c}{Uncorrected}                  &   \mc{3}{c}{Corrected}                    &                       \\
\hline
Category    &   NO. &   {\small Pred.}   &   {\small Frac.1}  &   NO. &   {\small Pred.}   &   {\small Frac.1}  &   NO. &   {\small Pred.}   &   {\small Frac.1}  \\
\hline
0.0-0.1   &   276 &   0.005    &   0.16    &   125 &   0.04    &   0.09    &   187 &   0.03    &   0.03    \\
0.1-0.2 &   14  &   0.14    &   0.36    &   61  &   0.15    &   0.10    &   46  &   0.15    &   0.26    \\
0.2-0.3 &   2   &   0.26    &   0.00    &   44  &   0.24    &   0.27    &   39  &   0.24    &   0.23    \\
0.3-0.4 &   10  &   0.35    &   0.80    &   39  &   0.35    &   0.28    &   17  &   0.34    &   0.35    \\
0.4-0.5 &   3   &   0.45    &   1.00    &   31  &   0.46    &   0.52    &   15  &   0.44    &   0.20    \\
0.5-0.6 &   5   &   0.52    &   0.60    &   35  &   0.55    &   0.63    &   27  &   0.56    &   0.63    \\
0.6-0.7 &   7   &   0.65    &   0.43    &   37  &   0.65    &   0.59    &   21  &   0.66    &   0.81    \\
0.7-0.8 &   5   &   0.75    &   0.60    &   42  &   0.74    &   0.86    &   26  &   0.76    &   0.85    \\
0.8-0.9 &   11  &   0.85    &   0.64    &   68  &   0.86    &   0.79    &   55  &   0.85    &   0.91    \\
0.9-1.0 &   267 &   0.99    &   0.84    &   118 &   0.96    &   0.93    &   167 &   0.97    &   0.95    \\
\hline
\end{tabular}
\end{center}
\end{slide}
%-------------------------------------------------------slide10
\begin{slide}
\tb The Markov chain traces of $\log(\alpha)$\tn
\centerline{\tiny Dashed line: Uncorrected method, Solid line: Corrected method, Horizonal line: the true value}
\begin{center}
\includegraphics[scale=0.3,angle=-90]{plot-logr400.ps}
\end{center}
\end{slide}

\begin{slide}
\tb Comparison of computational time (seconds) \tn
\begin{table}[htp]
\begin{center}
\begin{tabular}
{c|ccccc|c} \hline
        Number of Features&1&10&100&1000&2000&10000\\
        Fraction of Selection&0.01\%&0.1\%&1\%&10\%&20\%&100\%\\
\hline
    Corrected &4597& 5246&6515&12134&17473&\\
    Uncorrected &5& 48&479&4780&9544&48368\\
\hline
\end{tabular}
\end{center}
\end{table}
Note: these times are for an implementation in R. 
\end{slide}
%-------------------------------------------------------slide10
\begin{slide}
\tb Illustration on a real data set \tn
\begin{itemize}
\item {\bf Data sets}: Colon cancer data set, which has 62 cases and 2000 features. Divided into 10 smaller datasets, each with 200 randomly chosen features. We transformed the features to binary by thresholding at the medians. Five of the 200 features were selected based on the absolute correlation. 
\item {\bf Assessment}: We used 10-fold cross-validation to compare the prediction performance of corrected and uncorrected methods. We compared the Mean Square Error (MSE) of the predictive probabilities from the true responses. The MSE values are shown by the following table:
\begin{table}
\tiny
\begin{center}
\begin{tabular}{c|cccccccccc}
\hline
Uncorrcted &.1324 &.1351 &.1655 &.1763 &.1525
            &.1696 &.1583 &.1432 &.1681&.1667 \\
Corrected   &.1294 &.1306 &.1621 &.1678 &.1403
            &.1625 &.1534 &.1480 &.1637 &.1668\\
Difference  &.0030  &.0045  &.0034  &.0085  &.0122
            &.0071  &.0050  &-.0048  &.0044 & -.0002\\
\hline
\end{tabular}
\end{center}
\end{table}
\item The paired t-test on the two rows of MSE values gives 
a p-value of 0.017, showing that our bias correction method improves prediction.
\end{itemize}
\end{slide}

\begin{slide}
\tb Conclusion and Future Work \tn
\begin{itemize}
\item We've proposed a correction method to avoid the bias from feature selection.
\item We've applied the method to binary naive Bayes models. The simulation results show that it does avoid the bias from feature selection and it is faster than using all features. The results from microarray datasets show that the corrected method improves the predictive performance.
\item The evaluation of the adjustment factor is difficult. For binary naive Bayes models, the method we used is fairly fast and precise. This method can be generalized to all discrete naive Bayes models.
\item We've also applied the correction method to binary mixture models and factor analysis models. Evaluation of the adjustment factor for these models is more difficult but still feasible.
\item Future work is needed to improve efficiency and extend the method to more models and other selection criteria.
\end{itemize}
\end{slide}

\ndc


==> tab_mix300.tex <==
\begin{tabular}
{@{}c|@{}rcc|@{}rcc|rcc|rcc@{}}
         & \multicolumn{6}{c|}{\bf  1 feature selected out of 10000 } & \multicolumn{6}{c}{\bf  10 features selected out of 10000 } \\[5pt] 
         & \multicolumn{3}{c}{Corrected} & \multicolumn{3}{c|}{Uncorrected} & \multicolumn{3}{c}{Corrected} & \multicolumn{3}{c}{Uncorrected} \\[5pt] 
C & \mbox{~~~}\#\mbox{~} & \small{Pred} & \small{Actual} & \mbox{~~~}\#\mbox{~} & \small{Pred} & \small{Actual} & \mbox{~~}\#\mbox{~} & \small{Pred} & \small{Actual} & \mbox{~~}\#\mbox{~} & \small{Pred} & \small{Actual} \\[5pt] 
0 &    0 &    -- &    -- &    0 &    -- &    -- &    0 &    -- &    -- &  200 & 0.080 & 0.460 \\ 
1 &    0 &    -- &    -- &    0 &    -- &    -- &    0 &    -- &    -- &  424 & 0.158 & 0.502 \\ 
2 &    0 &    -- &    -- &    0 &    -- &    -- &   33 & 0.264 & 0.364 &   60 & 0.230 & 0.467 \\ 
3 &    0 &    -- &    -- & 1339 & 0.361 & 0.503 &  652 & 0.348 & 0.492 &  450 & 0.338 & 0.524 \\ 
4 & 2000 & 0.449 & 0.517 &    0 &    -- &    -- &  948 & 0.447 & 0.526 &   87 & 0.445 & 0.506 \\ 
5 &    0 &    -- &    -- &  661 & 0.576 & 0.546 &  294 & 0.543 & 0.520 &  239 & 0.562 & 0.540 \\ 
6 &    0 &    -- &    -- &    0 &    -- &    -- &   69 & 0.631 & 0.681 &  208 & 0.646 & 0.514 \\ 
7 &    0 &    -- &    -- &    0 &    -- &    -- &    4 & 0.719 & 0.750 &  184 & 0.759 & 0.511 \\ 
8 &    0 &    -- &    -- &    0 &    -- &    -- &    0 &    -- &    -- &  148 & 0.838 & 0.622 \\ 
9 &    0 &    -- &    -- &    0 &    -- &    -- &    0 &    -- &    -- &    0 &    -- &    -- \\ 
\end{tabular}

\vspace*{0.45in}
\begin{tabular}
{@{}c|@{}rcc|@{}rcc|rcc|rcc@{}}
         & \multicolumn{6}{c|}{\bf  100 features selected out of 10000 } & \multicolumn{6}{c}{\bf  1000 features selected out of 10000 } \\[5pt] 
         & \multicolumn{3}{c}{Corrected} & \multicolumn{3}{c|}{Uncorrected} & \multicolumn{3}{c}{Corrected} & \multicolumn{3}{c}{Uncorrected} \\[5pt] 
C & \mbox{~~~}\#\mbox{~} & \small{Pred} & \small{Actual} & \mbox{~~~}\#\mbox{~} & \small{Pred} & \small{Actual} & \mbox{~~}\#\mbox{~} & \small{Pred} & \small{Actual} & \mbox{~~}\#\mbox{~} & \small{Pred} & \small{Actual} \\[5pt] 
0 &    0 &    -- &    -- &  778 & 0.035 & 0.441 &    0 &    -- &    -- & 1013 & 0.018 & 0.399 \\ 
1 &    0 &    -- &    -- &  190 & 0.147 & 0.542 &    4 & 0.168 & 0.250 &   72 & 0.150 & 0.556 \\ 
2 &    4 & 0.273 & 0.250 &  100 & 0.245 & 0.550 &  118 & 0.273 & 0.297 &   46 & 0.244 & 0.522 \\ 
3 &  425 & 0.371 & 0.435 &   82 & 0.348 & 0.524 &  507 & 0.358 & 0.367 &   36 & 0.351 & 0.417 \\ 
4 & 1292 & 0.448 & 0.522 &   79 & 0.451 & 0.532 &  719 & 0.451 & 0.522 &   40 & 0.445 & 0.550 \\ 
5 &  268 & 0.528 & 0.634 &   77 & 0.553 & 0.610 &  515 & 0.544 & 0.654 &   25 & 0.540 & 0.600 \\ 
6 &   11 & 0.620 & 0.455 &   80 & 0.648 & 0.487 &  130 & 0.627 & 0.762 &   38 & 0.644 & 0.737 \\ 
7 &    0 &    -- &    -- &   88 & 0.757 & 0.545 &    7 & 0.722 & 0.286 &   48 & 0.753 & 0.688 \\ 
8 &    0 &    -- &    -- &  140 & 0.854 & 0.579 &    0 &    -- &    -- &   66 & 0.854 & 0.561 \\ 
9 &    0 &    -- &    -- &  386 & 0.958 & 0.606 &    0 &    -- &    -- &  616 & 0.974 & 0.677 \\ 
\end{tabular}

\vspace*{0.45in}
\begin{tabular}[t]
{@{}c|@{}rcc@{}}
         & \multicolumn{3}{c}{\bf Complete data} \\[5pt] 
C & \mbox{~~~}\#\mbox{~} & \small{Pred} & \small{Actual} \\[5pt] 
0 &    0 &    -- &    -- \\ 
1 &    0 &    -- &    -- \\ 
2 &    0 &    -- &    -- \\ 
3 &    0 &    -- &    -- \\ 
4 & 2000 & 0.443 & 0.517 \\ 
5 &    0 &    -- &    -- \\ 
6 &    0 &    -- &    -- \\ 
7 &    0 &    -- &    -- \\ 
8 &    0 &    -- &    -- \\ 
9 &    0 &    -- &    -- \\ 
\end{tabular}

